Task Adaptive Parameter Sharing for Multi-Task Learning

Adapting pre-trained models with broad capabilities has become standard practice for learning a wide range of downstream tasks. The typical approach of fine-tuning different models for each task is performant, but incurs a substantial memory cost. To efficiently learn multiple downstream tasks we introduce Task Adaptive Parameter Sharing (TAPS), a general method for tuning a base model to a new task by adaptively modifying a small, task-specific subset of layers. This enables multi-task learning while minimizing resources used and competition between tasks. TAPS solves a joint optimization problem which determines which layers to share with the base model and the value of the task-specific weights. Further, a sparsity penalty on the number of active layers encourages weight sharing with the base model. Compared to other methods, TAPS retains high accuracy on downstream tasks while introducing few task-specific parameters. Moreover, TAPS is agnostic to the model architecture and requires only minor changes to the training scheme. We evaluate our method on a suite of fine-tuning tasks and architectures (ResNet, DenseNet, ViT) and show that it achieves state-of-the-art performance while being simple to implement.

==> Tables/Sparsity.tex <==
\begin{table}[]
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
{\color[HTML]{333333}} & Flowers                                              & Cars    & Sketches & WikiArt & CUBS    \\ \hline
Sparsity                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}21.4} & 31.1 & 33.7 & 32.1 &  33.3
\end{tabular}
\label{tab:sparsity}
\caption{Percent sparsity given the respective hyper-parameters.}
\end{table}

==> Tables/Transformers.tex <==
\begin{table}
\small
\begin{tabular}{llllll}
\toprule
                       & \Flowers & \Wiki & \Sketch & \Cars & \CUB \\ \hline
Fine-Tuning            & 0.67           & 17.44   & 18.09  & 10.79         & 11.11     \\
DWS                    & 0.88           & 17.72   & 17.82  & 11.32         & 11.58     \\
%Addl. Parameters(\%) & 41.28          & 30.42   & 24.07  & 26.15         & 41.28     \\ \bottomrule
\end{tabular}
\caption{Performance of DWS and fine-tuning using a ViT architecture on different datasets. \hao{which ViT model do you use here (timm model id)? Is the image input size 224 or 384?}}
\label{tab:transformer}
\end{table}

==> Tables/adashare_resnet34_policy_incremental.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\small
\centering
\label{tab:adashare_policy_incre}
\begin{tabular}{r|c|r|r|r|r|r|r|r|r}
% \scriptsize
\multicolumn{1}{l|}{Stage} & Block                                   & \multicolumn{1}{l|}{\#size} & \multicolumn{1}{l|}{param \%} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{real}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{paint.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{quick.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{clip.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{infor.}} & \multicolumn{1}{l}{\rotatebox[origin=c]{270}{sketch}} \\ \hline
\multirow{3}{*}{1}          & \multirow{3}{*}{Conv(3x3,64)*2*3}  & \multirow{3}{*}{56x56} & 0.34                           & 1                         & 1                             & \textbf{0}                     & 1                            & 1                              & 1                  \\ \cline{4-10} 
                            &                                    &                        & 0.34                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                  \\ \cline{4-10} 
                            &                                    &                        & 0.34                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \hline
\multirow{4}{*}{2}          & \multirow{4}{*}{Conv(3x3,128)*2*4} & \multirow{4}{*}{28x28} & 1.02                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 1.36                           & 1                         & 1                             & \textbf{1}                     & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 1.36                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 1.36                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \hline
\multirow{6}{*}{3}          & \multirow{6}{*}{Conv(3x3,256)*2*6} & \multirow{6}{*}{14x14} & 4.09                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 5.46                           & \textbf{0}                & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \hline
\multirow{3}{*}{4}          & \multirow{3}{*}{Conv(3x3,512)*2*3} & \multirow{3}{*}{7x7}   & 16.38                          & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                    &                        & 21.84                          & 1                         & 1                             & 1                              & 1                            & 1                              & 1                  \\ \cline{4-10} 
                            &                                    &                        & 21.84                          & 1                         & 1                             & 1                              & 1                            & \textbf{0}                     & 1                           \\ \hline
\end{tabular}
\caption{\textbf{The sampled policy of AdaShare's learned in the incremental MTL setting on DomainNet}. The number 0 in each cell refers to whether the block is skipped.
The total number of parameters are 5.73x as no layers are skipped by all datasets.}
\end{table*}

==> Tables/adashare_resnet34_policy_joint.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\small
\centering
\label{tab:adashare_policy_joint}
\begin{tabular}{r|c|r|r|r|r|r|r|r|r}
% \scriptsize
\multicolumn{1}{l|}{Stage} & Block                                   & \multicolumn{1}{l|}{\#size} & \multicolumn{1}{l|}{param \%} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{real}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{paint.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{quick.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{clip.}} & \multicolumn{1}{l|}{\rotatebox[origin=c]{270}{infor.}} & \multicolumn{1}{l}{\rotatebox[origin=c]{270}{sketch}} \\ \hline
\multirow{3}{*}{1}          & \multirow{3}{*}{Conv(3x3,64)x2x3}      & \multirow{3}{*}{56x56} & 0.34                           & 1                         & 1                             & \textbf{0}                     & 1                            & 1                              & \textbf{0}                  \\ \cline{4-10} 
                            &                                        &                        & 0.34                           & 1                         & 1                             & 1                              & 1                            & 1                              & \textbf{0}                  \\ \cline{4-10} 
                            &                                        &                        & 0.34                           & 1                         & 1                             & 1                              & 1                            & 0                              & 1                           \\ \hline
\multirow{4}{*}{2}          & \multirow{4}{*}{Conv(3x3,128)x2x4}     & \multirow{4}{*}{28x28} & 1.02                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 1.36                           & 1                         & 1                             & \textbf{0}                     & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 1.36                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 1.36                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \hline
\multirow{6}{*}{3}          & \multirow{6}{*}{Conv(3x3,256))x2x6} & \multirow{6}{*}{14x14} & 4.09                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 0                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 5.46                           & \textbf{0}                & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 5.46                           & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \hline
\multirow{3}{*}{4}          & \multirow{3}{*}{Conv(3x3,512)x2x3}     & \multirow{3}{*}{7x7}   & 16.38                          & 1                         & 1                             & 1                              & 1                            & 1                              & 1                           \\ \cline{4-10} 
                            &                                        &                        & 21.84                          & 1                         & 1                             & 1                              & 1                            & 1                              & \textbf{0}                  \\ \cline{4-10} 
                            &                                        &                        & 21.84                          & 1                         & 1                             & 1                              & 1                            & 1                     & 1                           \\ \hline
\end{tabular}
\caption{\textbf{The sampled policy of AdaShare learned in the joint MTL setting on DomainNet}. The model is ResNet-34. 
The number 0 in each cell refers to whether the block is skipped. 
The total number of parameters are 1$x$ as no layers are skipped by all datasets.}
\end{table*}

==> Tables/dataset.tex <==
\begin{table*}[!h]
\centering
\renewcommand{\arraystretch}{1.25}
\label{tab:dataset}
\footnotesize
\begin{tabular}{llrrr}
\toprule
        Benchmark & Dataset                 & & Classes   & Training      & Test  \\ \hline
         & Oxford Flowers~\cite{flowers}      & 102       & 2,040         & 6,149   \\
         & CUB-Birds 200-2011~\cite{birds}   & 200       & 5,994         & 5,794   \\
         & FGVC Aircrafts~\cite{aircrafts}  & 100       & 6,667         & 3,333   \\
         & Stanford Cars~\cite{cars}       & 196       & 8,144         & 8,041   \\
        %  Stanford Dogs~\cite{dogs}       & fine-grained object recog.  & 120       & 12,000        & 8,580   \\
        %  MIT Indoor-67~\cite{indoor67}       & scene classification             & 67        & 5,360         & 1,340   \\
        %  Caltech-256-60~\cite{caltech256}      & general object recog.       & 256        & 15,360         & 15,189\\\hline
        %  iNaturalist 2017~\cite{inat} & fine-grained object recog. & 5,089      & 665,571 & 9,599\\
        %  Place365~\cite{zhou2018places}       & scene classification              & 365          & 1,803,460   & 36,500 \\
         \bottomrule
\end{tabular}
\caption{\small Datasets statistics.
% For the Aircraft and Flower dataset, we combined the original training set and validation set and evaluated on the test set. 
% \AR{Why are we listing datasets we dont even use here?}\hao{we can comment those lines we don't need}
}
\end{table*}

==> Tables/densenet-121-params.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lccccc}
\toprule
 & \Flowers & \Wiki & \Sketch  & \Cars & \CUB\\
\midrule
Fine-Tuning & 4.40 & 23.04  & 18.93 & 10.46	 & 17.42	 \\
Piggyback & 5.31 & 29.56 & 20.30 & 10.87 & 19.50 \\ 
%Piggback GIT & 4.91 & 29.33 & 20.05 & 10.62 & 19.24 \\
\midrule 
DWS  &  4.22 & 26.40 & 19.77	 &  11.97 & 0.1912
\\
Addl. Parameters &80.16  & 41.22 &58.48  & 50.36  &  47.11\\
\bottomrule

\end{tabular}
\caption{Performance of different method using a Densnet-121 model on different datasets. Shown in the table is the classification error for different methods across different datasets. For our method, the fine-tuning paragon, we report the average error over three runs of the method. \avinash {What else comparisons needs to go here?. The task distance correlation might be a little bit off key here as there are differen learning rates. } }
\label{tab:basedensenet}
\end{table*}

==> Tables/densenet-121.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lccccc}
\toprule
 & \Flowers & \Wiki & \Sketch  & \Cars & \CUB\\
\midrule
Fine-Tuning & 4.40 & 23.04  & 18.93 & 10.46	 & 17.42	 \\
Piggyback & 5.31 & 29.56 & 20.30 & 10.87 & 19.50 \\ 
%Piggback GIT & 4.91 & 29.33 & 20.05 & 10.62 & 19.24 \\
\midrule 
DWS  &  4.22 & 26.40 & 19.77	 &  11.97 & 0.1912
\\
%Addl. Parameters &80.16  & 41.22 &58.48  & 50.36  &  47.11\\
\bottomrule

\end{tabular}
\caption{Performance of different method using a Densnet-121 model on different datasets. Shown in the table is the classification error for different methods across different datasets. For our method, the fine-tuning paragon, we report the average error over three runs of the method. \avinash {What else comparisons needs to go here?. The task distance correlation might be a little bit off key here as there are differen learning rates. } }
\label{tab:basedensenet}
\end{table*}

==> Tables/old_accuracy_sparsity.tex <==
\begin{table}[]
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\toprule
{\color[HTML]{333333} } & Flowers                                            & Cars  & Sketches & WikiArt & CUBS \\ \midrule
DWS                           & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}95.71} & 91.20 & 80.31    & 78.9    & 83.7\\
\bottomrule
\end{tabular}
\caption{Accuracy for best model for each downstream task.}
\end{table}

==> Tables/param_count.tex <==
\begin{table*}[]
\caption{Paramters used for different methods.}
\begin{tabular}{llllll}
Method & reported & Parameter factor & Data-type norm count \\
Piggyback & $1 + \frac{k-1} {32}$ & $\frac{n + kn + (k+1) b}{k+b}$ & $\frac{32n + k + (k+1) * b*32} {32n+32b}$ \\ 
 Spottune &  $k+1$ & $\frac{(k+1)n + p + (k+1)b}{k(n+b)}$ &  $\frac{(k+1)n + p + (k+1)b}{k(n+b)}$

\end{tabular}
\end{table*}


\begin{table*}[]
\caption{Paramters used for different methods.}
\begin{tabular}{llllll}
Method & reported & Parameter factor & Data-type norm count \\
Piggyback & $1 + \frac{k-1} {32}$ & $k$ & $ 1+ \frac{k-1} {4}$ & 2.25 & 3.25. 
\\ 
\end{tabular}
\end{table*}

==> Tables/resnet-hpo.tex <==

\begin{table}[]
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
{\color[HTML]{333333} Method} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}Flowers} & Cars                                            & Sketches                                        & WikiArt                                         & CUBS                                           \\ \hline
lr                 & .01                                                 & .01                                             & .005                                            & .005                                            & .005                                          \\
$\lambda$                        & .1                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}.1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}.1} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}.1}
\end{tabular}
\caption{Hyper-parameters for each result. Weight decay is 0 and momentum is .9 for all experiments. Batch Size is 32, and epochs trained is 30. Values searched for learning rate: [.01, .005, .001, .0005]. Values searched for $\lambda$: [.1, .3].}
\hao{hyperparameter search space needs to be consistent with previous training details.}
\end{table}


==> notes.tex <==
%\hao{checklist of the topics we mentioned in the main paper that will be discussed in the supplementary materials:
%\begin{itemize}
% \item \st{line 402: ``Details about the datasets and their augmentation are in the \Suppmat{}."}
% \item \st{line 416: ``The individual parameter counts are available in
% Supp. Material."}
% \item \st{line 458:``The details of the training (DenseNet-121 and Transformers) for these settings can be found in the Supp. Material"}
% \item \st{line 482: ``We report the number of parameters used for
% each task in the Supp. Material'}
%\item line 503: ``A detailed figure of the task-specific layers for this task can be %found in the Supp. Material."
%\item line 516: ``we also see a drop 2.77\% in average accuracy across the datasets %(see Supp. Material for details)"
% \item \st{line 532: ``we use the ViT-S/16 model [42] (see Supp. Material for the training details)"}
% \item \st {line 718: ``We also include full fine-tuning as a baseline. Detailed training settings can be found in the Supp. Material"}
\end{itemize}
%

